The COSMOS-Web Lens Survey (COWLS) I: Discovery of >100 high redshift strong lenses in contiguous JWST imaging

We present the COSMOS-Web Lens Survey (COWLS), a sample of over 100 strong lens candidates from the $0.54$\,deg$^2$ COSMOS-Web survey, discovered using exquisite James Webb Space Telescope (JWST) imaging across four wavebands. Following two rounds of visual inspection, over 100 candidates were ranked as `high confidence' or `likely' by at least $50\%$ of inspectors. The COWLS sample has several notable properties: (i) magnified source galaxies spanning redshifts $z \sim 0.1$ to $z \sim 9$, which therefore extend into the epoch of reionisation; (ii) the highest-redshift lens galaxies known, pushing galaxy density profile evolution studies beyond $z \sim 2$; (iii) all lenses are distributed within a contiguous $0.54$\,deg$^2$ region, allowing for joint strong and weak lensing analyses; and (iv) a subset exhibits lensed source emission ray-traced near the lens galaxy centers, enabling studies of supermassive black holes and dust absorption. A key innovation of our approach is the use of lens modelling to aid in identifying lenses that may otherwise be missed. This paper is accompanied by the first COWLS public release, providing JWST NIRCam imaging in four bands, lens models, pixelized source reconstructions and lens redshift estimates : https://github.com/Jammy2211/COWLS_COSMOS_Web_Lens_Survey

==> scrap.tex <==
James Nightingale,
Guillaume Mahler, 
Jacqueline McCleary,
Qiuhan He,
Natalie B. Hogg,
Aristeidis Amvrosiadis,
Ghassem Gozaliasl,
Wilfried Mercier,
Diana Scognamiglio,
Edward Berman,
Gavin Leroy,
Daizhong Liu
Richard J. Massey,
Marko Shuntov,
Maximilian von Wietersheim-Kramsta, 
Maximilien Franco,
Louise Paquereau,
Olivier Ilbert,
Natalie Allen,
Sune Toft, 
Hollis B. Akins,
Caitlin M. Casey,
Jeyhan S. Kartaltepe,
Anton M. Koekemoer,
Henry Joy McCracken,
Jason D. Rhodes,
Brant E. Robertson,
Nicole E. Drakos,
Andreas L. Faisst,
Shuowen Jin
